Analysis of Knuth's Sampling Algorithm D and D'

In this research paper, we address the Distinct Elements estimation problem in the context of streaming algorithms. The problem involves estimating the number of distinct elements in a given data stream $\mathcal{A} = (a_1, a_2,\ldots, a_m)$, where $a_i \in \{1, 2, \ldots, n\}$. Over the past four decades, the Distinct Elements problem has received considerable attention, theoretically and empirically, leading to the development of space-optimal algorithms. A recent sampling-based algorithm proposed by Chakraborty et al.[11] has garnered significant interest and has even attracted the attention of renowned computer scientist Donald E. Knuth, who wrote an article on the same topic [6] and called the algorithm CVM. In this paper, we thoroughly examine the algorithms (referred to as CVM1, CVM2 in [11] and DonD, DonD' in [6]. We first unify all these algorithms and call them cutoff-based algorithms. Then we provide an approximation and biasedness analysis of these algorithms.

==> cutoffalgo.tex <==
\section{Cutoff and Refuse-based Algorithm}
We introduce a modification to the cutoff-based algorithm, allowing for the possibility of refusing to select an element even if it satisfies the current cutoff. This adjustment is typically employed when the size of the list reaches its limit or exceeds it. The final step of the modified algorithm carried out at time $t$, occurs after all previous steps, specifically after step 4 of the cutoff-based algorithm. At this stage, we have $L_t = \textsc{Filter}(L'_t, p_t)$ (resulting from step 4).
\begin{enumerate}
	\item[Step 5] If $\refute(L_t) = 1$, then $L_t = L_t \setminus {(a_t, q_t)}$ (refusing to include the current element even if it passed the $\textsc{Filter}$ operation).
\end{enumerate}
This step is similar to the "abort" operation in CVM1 but with a crucial difference. In CVM, once the abort occurs, the estimation process is terminated and the event is considered an error. In our case, however, we continue processing until the last element.

\begin{definition}
	Let $\algo$ be a cutoff-based algorithm with $s$ as a bucket limit. Let 
	\begin{center}
		$\refute(L_t) = 1$ if and only if $|L_t| \geq s+1$ 
	\end{center}
	(this implies that $|L'_{t}| = s+1$ and no element is removed after the $\textsc{Filter}$ step). We write $\algo_{\refute}$ to denote the algorithm which first runs steps of $\algo$ and then applies the above $\refute$ step (for all $t$). We also call it a refuse-adjoined version of the original cutoff-based algorithm.
\end{definition}
Now we make the following useful observations:
\begin{enumerate}
	\item Note that a refuse-adjoined algorithm behaves the same as that without refuse if the $\refute$ function always returns 0. 
	
	\item Clearly a refuse-based algorithm is not fair. However, it may satisfy the fairness property at the end 
	if no refuse happens at any one of the time in $\mathcal{F}_m$. More formally, let $E_t$, $t \in \mathcal{F}_m$, be the event that 
	$\refute$ returns 1. Now,  if $\algo$ is an $(\epsilon, \delta)$-approximation then $\algo_{\refute}$ is an $(\epsilon, \delta')$-approximation where $\delta' = \delta + \sum_{t \in \mathcal{F}_m}\pr(E_t)$.
\end{enumerate}

\begin{theorem}
	Let $\algo$ be a {\em decreasing cutoff-based}, {\em good} sampling algorithm which uses a {\em linear score distribution} $D$ (over $\Omega$). Moreover, we assume it never aborts or returns $p_m \leq \min \Omega$. Then, the final estimate $|L_m|/p_m$ of $\algo_{\refute}$ is an $\delta'$-biased estimate of $F_0$ where $\delta' = \sum_{t \in \mathcal{F}_m}\pr(E_t)$ where $E_t$'s are the events described above.
\end{theorem}

\proof The proof follows exactly in the same line of Theorem~\ref{thm:unbiased}.
For all $a_t \in A$ with $t \in \mathcal{F}_m$ such that $\refute$ returns 0 at time $t$, then 
$\ex(I_a/p_m ~|~ q^m_{-j}) = 1,~~ \forall q^m_{-j}.$
Otherwise, if $\refute$ returns 1, then $\ex(I_a/p_m ~|~ q^m_{-j}) = 0,~~ \forall q^m_{-j}.$ So, $|\ex(|L_m|/p_m)- |A|| \leq E(|R|)$ where $R$ denotes the set of all those $t \in \mathcal{F}_m$ for which the element $a_t$ was refused. Hence, by linearity, we have our result. \qed  


\begin{cor}
	Let $0 < \epsilon, \delta \leq 1$, $n' = \min\{n, m\}$ and $s = 12\log\frac{4n'}{\delta} +\frac{6}{\epsilon^2} \log\frac{8}{\delta}$.
	Then $\mathrm{CVM2}_{\refute}$ is (i) $\delta$-biased and (ii) $(\epsilon, \delta)$-approximation $F_0$ estimation algorithm. The space complexity of the algorithm is 
	$$\mathcal{O}(\log^2 n') + \mathcal{O}(\epsilon^{-2} \log \delta^{-1}\log n').$$
	Moreover, if we choose $s =  \frac{12}{\epsilon^2} \log\frac{8m}{\delta}$ then it returns $(\epsilon, \delta)$-approximation for all time $t \in [m]$ (also known as constant tracking algorithm). 
\end{cor}


\begin{algorithm}\label{algo2}
	Initialize $p_0 \leftarrow 1 $; $L_0 \leftarrow \emptyset $; \\
	%    thresh $ \leftarrow \mathsf{th}$\\
	\For{$t=1$ \KwTo $m$}{
		$R_{t,0} \sim Ber(p_{t-1})$ \\
		\If{$R_{t, 0} = 0$}{$L'_t = \textsc{Remove}(L_{t-1}, a_t)$}
		\Else{$L'_t = \textsc{Remove}(L_{t-1}, a_t) \cup \{(a_t, p_{t-1}) \}$}
		\If{$|L'_t| =  s+1$}{
			$(R_{t,a} : a \in \set(L'_t)) \iid Ber(1/2)$ \\
			$p_t \leftarrow p_{t-1}/2$ \\
			$L_t = \{ (a, p_t): (a, p) \in L'_t, R_{t, a} = 1\}$ \\
			\If{$|L_t| = |L'_t|$}{ $L_t \leftarrow \textsc{Remove}(L_{t}, a_t)$}
		}       
	}
	\KwRet{$\frac{|L_m|}{p_m}$}
	\caption{$\mathrm{CVM2}_{\refute}$. This behaves same as CVM1. Instead of Abort, we refute the element $a_t$ in keeping the list (same as refute-adjoined version of CVM2.}
\end{algorithm}

\section{Estimate for Stream of Sets}\label{sec:stream:set}
Now we consider a variant of Delphic setup.


%\textcolor{red}{Write THE DELPHIC SETUP.. }


\begin{definition}[Delphic family]
	\label{def:delphic}
	Let $\Omega$ be a discrete universe. A set $S \subseteq \Omega$ is considered to be a Delphic family\footnote{It has been observed that every Delphic set can be represented by a circuit of size $O(\log |\Omega| \log \log |\Omega|)$.} if the following queries can be performed in $O(\log |\Omega|)$ time:
	\begin{description}
		\item[Membership] Given any $x \in \Omega$, determine whether $x \in S$.
		\item[Cardinality] Find the size of $S$, denoted as $|S|$.
		\item[Sampling] Generate a uniform random sample from $S$.
	\end{description}
\end{definition}

We consider a slightly different variant of Delphic family where we replace the item Sampling with Picking if we have an ordering on the set $S$:

\begin{description}
	\item[Picking] Given a set $ S $ and a positive integer $ i \leq |S| $, we can pick the $ i$-th element of $ S$.
\end{description}








% In addition to all these, we also have one more additional subroutine which can draw $i$th element of the set $S$ where $i \leq |S|$. 

Here we assume that the elements of the set $S$ have some implicit ordering and based on the ordering it is now efficient to draw the $i$th element for any $i$. Note that this is indeed true for a cuboid sets $S := [a_1.. b_1] \times \cdots [a_d.. b_d]$ where $1 \leq a_i \leq b_i \leq n$. This property can be obtained for some other structures of sets also. With this, we now define how to estimate of the distinct element problem for a stream of sets $\mathcal{S} = (S_1, \ldots, S_m)$. 


\noindent Upon receiving a set $S_t$ at time $t \in [m]$, the algorithm follows the following steps:
\begin{enumerate}
	
	
	\item Let $L'_t = \textsc{Remove}(L_{t-1}, S_t)$ denote the intermediate list (we can remove elements of $S_t$ by using the membership oracle). 
	
	\item $C = 0$, $p_t = p_{t-1}$. 
	
	\item Do the following steps while $C \leq |S_t|$
	
	\begin{itemize}
		\item Pick $C$th element, $x$ from $S_t$ and add in the list $L'_t \leftarrow L'_t \cup (x, p_{t})$. 
		
		\item If $|L'_t| = s+1$ then sample w.p. 1/2 elements of $L'_t$ and $p_t \leftarrow p_{t}/2$, If it still has the same size, we refuse to add $x$ and continue. 
		
		\item Sample $i \sim Geo(p_{t})$ and $C \leftarrow C + i$  
	\end{itemize}
	
	
	%This step is common in all sampling-based algorithms.
	
	% \item Compute the updated cutoff value $p_t$ using the cutoff update function $C$:
	% $$p_t := C(L'_{t}, p_{t-1})$$
	% Here we assume that the pair $(a_t, q_t)$ is marked in the last $L'_t$ so that the cutoff update function can use it explicitly. 
	
	% \item Construct the list $L_t = \textsc{Filter}(L'_{t}, p_t)$.
	
\end{enumerate}
\noindent After processing all elements, a final estimate $\hat{F} := |L_m|/p_m$. We denote this algorithm as $\algo_{DEL}$\label{algo:our:set}. \medskip

\begin{theorem}\label{thm:set:stream}
	Let $0 < \epsilon, \delta \leq 1$, $n' = \min\{n, m\}$ and $s = 12\log\frac{4n'}{\delta} +\frac{6}{\epsilon^2} \log\frac{8}{\delta}$.
	Then $\algo_{DEL}$ is (i) $\delta$-biased and (ii) $(\epsilon, \delta)$-approximation $F_0$ estimation algorithm. The space complexity of the algorithm is 
	$$\mathcal{O}(\log^2 n') + \mathcal{O}(\epsilon^{-2} \log \delta^{-1}\log n').$$
	Moreover, if we choose $s =  \frac{12}{\epsilon^2} \log\frac{8m}{\delta}$ then it returns $(\epsilon, \delta)$-approximation for all time $t \in [m]$ (also known as constant tracking algorithm). 
\end{theorem}


% \section{Multiple Cutoff based Sampling Algorithms}
% We now generalize this to multiple cutoff based algorithms. This is basically running $\ell$ such algorithms of the above kind (may be in a dependent way). However, we would like to keep one element in at most one such cutoff based algorithm.  More formally, at time $t$, we have a tuple of lists $\mathcal{L}_{t-1} := (L^{(1)}_{t-1}, \ldots, L^{(\ell)}_{t-1})$ and a tuple of cutoffs $\mathcal{C}_{t-1} := (c^{(1)}_{t-1}, \ldots, c^{(\ell)}_{t-1})$. We initialize all lists empty and set all cutoff values $-1$ (similar to the single cutoff based algorithm). \medskip

% \noindent\underline{{\bf Multiple Cutoff Based Algorithm}} \\
% On receiving an element $a_t$, at time $t$, we perform the following steps:
% \begin{enumerate}
	%     \item Remove $(a, q)$ from $L^{(i)}_{t-1}$ if there is any such element for some $i$ and $q$; 
	% \item Sample an independent score $q_t$ following a specified distribution $\mathcal{D}$. 
	% \item Compute the updated cutoff value using the cutoff update function $C^*$:
	% $$(\mathcal{C}_{t}, i_t) := C^*(\mathcal{C}_{t-1}, \mathcal{L}_{t-1}, (a_t, q_t)).$$ 
	% Note that the cutoff function also decides an integer $i_t \in [\ell]$ which describes in which list we would like to include the current element. 
	% \item For all $i \neq i_t$, we define \[L_t^{(i)} := \{ (a, q) \in L_{t-1}^{(i)} : q > c_t^{(i)} \}\]
	% and for $i = i_t$, we define 
	% \[L_t^{(i_t)} := \{ (a, q) \in L_{t-1}^{(i)} \cup \{(a_t, q_t)\} : q > c_t^{(i_t)}\}.\]
	% \end{enumerate}
% A variable cutoff can apply a post-processing (after all elements have been processed) to look like a single cutoff based algorithm. It finally defines a final cutoff $c^*$ and then defines a final list 
% \[L^* := \{ (a, q) \in L_m^{(i)} : q > c^*, i \in [\ell] \}.\]
% Now, $L^*$ and $c^*$ behave like a result of single cutoff based algorithm (however, it is more stronger as it may not be realized by a single cutoff algorithm). 
